Prime Factorization Using Quantum Variational Imaginary Time Evolution

The road to computing on quantum devices has been accelerated by the promises that come from using Shor's algorithm to reduce the complexity of prime factorization. However, this promise hast not yet been realized due to noisy qubits and lack of robust error correction schemes. Here we explore a promising, alternative method for prime factorization that uses well-established techniques from variational imaginary time evolution. We create a Hamiltonian whose ground state encodes the solution to the problem and use variational techniques to evolve a state iteratively towards these prime factors. We show that the number of circuits evaluated in each iteration scales as O(n^{5}d), where n is the bit-length of the number to be factorized and $d$ is the depth of the circuit. We use a single layer of entangling gates to factorize several numbers represented using 7, 8, and 9-qubit Hamiltonians. We also verify the method's performance by implementing it on the IBMQ Lima hardware.

==> sections/vqe.tex <==
\section{Comparison against VQE}

\begin{figure}[H]
    \centering
    \includegraphics[height=0.30\textwidth]{figures/var_circuit_1.png}
    \caption{Generalized 3-layer VQE ansatz used for optimization. The circuit parameters have been randomly initialized.}
    \label{fig:var_circuit_1}
\end{figure}

\begin{figure}[H]
    \begin{subfigure}[b]{0.50\textwidth}
        \includegraphics[width=\linewidth]{simulation-graphs/5_VQE.png}
        \caption{Amplitude of correct solution for various 5-qubit VQE simulations.}
        \label{fig:5_VQE}
    \end{subfigure}
    \begin{subfigure}[b]{0.50\textwidth}
        \includegraphics[width=\linewidth]{simulation-graphs/7_VQE.png}
        \caption{Amplitude of correct solution for various 7-qubits VQE simulations.}
        \label{fig:7_VQE}
    \end{subfigure}
    \caption{Numerical simulations of VQE for 5- and 7-qubit factorization examples. The vertical axis indicates the amplitude of the solution in the computational basis and the horizontal axis indicates the number of iterations made. The curves in each subplot, show how the amplitude of the solution corresponding to various numbers increase with iterations. The amplitude threshold has been set to 0.85}
    \label{fig:VQE_simulations}
\end{figure}


Variational quantum eigensolver (VQE) is yet another quantum-classical hybrid algorithm that stands as a potential candidate for solving optimization problems. Problems in quantum chemistry that solve for the ground state and its energy can be well represented as an optimization problem of the mean energy of the Hamiltonian with the parameters of the state allowing for variations.  Here we compare the simulation results from VQE against that of QITE. We have studied the performance using 2 different ansatz: one using the circuit in figure \ref{fig:vqe_circref} and the other using a more generalized version of the same with $R_x$ gates included as shown in figure \ref{fig:var_circuit_1}. Figure \ref{fig:VQE_simulations} shows that as we increase the number of qubits, VQE no longer is able to converge on the right solution for most cases. For the 9 qubit case, the VQE solution was observed to not converge at all. We also observed the addition of $R_x$ in the generalized ansatz did not help with the convergence.



We attribute the inability to converge on a solution for the larger number of qubits to exploring a barren plateau for an extended number of iterations. For circuits that emulate real coefficients, we have the following optimization rule for VQE,



\begin{equation}\label{eq:VQE_upd}
    \dot{\theta_i} = \frac{d}{d\theta_i}(\bra{\psi(\vec{\theta})} H \ket{\psi(\vec{\theta)}}) = \frac{1}{2}\Re(\frac{d}{d\theta_i}(\bra{\psi(\vec{\theta})}H \ket{\psi(\vec{\theta)}})
\end{equation}

Notice that equation \ref{eq:VQE_upd} is similar to the updates made in QITE, if the matrix $M_{ij}$ were to be identity. We would like to infer that the updates made with nontrivial $M$ coefficients help solve the barren plateau issue that is commonly observed in VQE.

